Strongly Interacting Higgs Sector Without Technicolor

Several years ago, we proposed a modification of the Standard Model, in which the Higgs sector was stabilized by the addition of higher derivative operators, similar to Lee-Wick Electrodynamics. We studied this theory extensively, both using continuum Hamiltonian and path integral methods. We also reported detailed lattice studies of the higher derivative Higgs sector. In view of some recent revived interest in our original idea, we are providing here our extensive notes from the time period on this topic. The key results were already published in our papers at that time. The many additional details that we make available here were previously available only in Chuan Liu's UCSD Ph.D. thesis (1994). Very recently, our idea has been revived by other groups. In view of the renewed interest, and to perhaps correct some misconceptions in the literature, we are here making our original extensive notes available to the wider community.

==> bib.tex <==
\begin{thebibliography}{9}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%   Standard Bibliography File  %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%
%%%%%%%%%%%%%%  The Standard Model in General           
%%%%%%
\bibitem{wein} S.~Weinberg, Phys. Rev. Lett. 19, (1967) 1264. 
\bibitem{salam} A.~Salam, Elementary Particle Theory, Ed., N.~Svartholm,
                 Almquist and Wiksell, 1968.
\bibitem{glash} S.~L.~Glashow, Nucl. Phys. 22, (1961) 579.
\bibitem{quigg} B.~W.~Lee, C.~Quigg and H.~B.~Thacker, Phys. Rev. D16,
(1977) 1519.
%%%%%%
%%%%%%%%%%%%%%  The Higher Derivative Theory in General 
%%%%%%
\bibitem{ostro} M.~Ostrogradski, Mem. Ac. St. Petersbourg 4 (1850) 385.
\bibitem{podo} B.~Podolski, Phys. Rev. 62 (1942) 68;
               B.~Podolski and P.~Schwed, Rev. Mod. Phys. 20 (1948) 40.   
\bibitem{pv} W.~Pauli and F.~Villars, Rev. Mod. Phys. 21 (1949) 434
\bibitem{pais} A.~Pais and G.~E.~Uhlenbeck, Phys. Rev. 79 (1950) 145
\bibitem{lee} T.~D.~Lee and G.~C.~Wick, Nucl. Phys. B 9 (1968) 209; Phys.
Rev. D 2 (1970) 1033.
\bibitem{polk} R.~E.~Cutkosky, P.~V.~Landshoff, D.~I.~Olive and 
J.~C.~Polkinghorne, Nucl. Phys. B12 (1969) 281.
\bibitem{ghost} K.~Jansen, J.~Kuti, C.~Liu Phys. Lett. B 309 (1993) 119.
\bibitem{gross} D.~G.~Boulware and D.~J.~Gross, Nucl. Phys. B233 (1983)
1.
\bibitem{pauli} W.~Pauli, Rev. Mod. Phys. 15 (1943) 175.
\bibitem{simon} J.~Z.~Simon, Phys. Rev. D41 (1990)  3720.
\bibitem{scat}  J.~Kuti and C.~Liu, to be published. 
%%%%%%
%%%%%%%%%%%% Higher Derivative Gauge Theory and Gravity
%%%%%%
\bibitem{slav} A.~A.~Slavnov, Nucl.~Phys. B31 (1971) 301.
\bibitem{hawk} S.~W.~Hawking, Quantum field theory and quantum
statistics, eds. I.~A.~Batalin et al. (1987) p. 129.
\bibitem{stelle} K.~S.~Stelle, Phys. Rev. D16 (1977) 953.
\bibitem{tomb} E.~Tomboulis, Phys. Lett. B97 (1980) 77.
%%%%%%
%%%%%%%%%%%% Algorithms Development
%%%%%%
\bibitem{kenn} A.~D.~Kennedy and B.~Pendleton, Nucl. Phys. B (Proc.
Suppl.) 20 (1991) 118.
\bibitem{parisi} G.~Parisi, Progress in gauge field theory, ed. G.~'t~
Hooft et al. (Plenum, New York, 1984) 531.
\bibitem{batrouni} G.~Batrouni, G.~Katz, A.~Kronfeld, G.~P.~Lepage, P.~
Rossi, B.~Svetitsky and K.~Wilson, Phys. Rev. D32 (1985) 2736.
\bibitem{kogut} E.~Dagotto and J.~B.~Kogut, Nucl. Phys. B 290 (1987)
451. 
%%%%%%
%%%%%%%%%%%% Triviality in General
%%%%%%
\bibitem{landau} L.~D.~Landau, A.~A.~Abrikosov and I.~M.~Khalatnikov,
Doklady Akad. Nauk. USSR 95 (1954) 1177.
\bibitem{maiani} L.~Maiani, G.~Parisi and R.~Petronzio, Nucl. Phys. B136
(1978) 115.
\bibitem{dash} R.~Dashen and H.~Neuberger, Phys. Rev. Lett. 50 (1983)
1897.
%%%%%%
%%%%%%%%%%%% Higgs Mass Bound 
%%%%%%
\bibitem{hhiggs} K.~Jansen, J.~Kuti, C.~Liu Phys. Lett. B309 (1993) 127.
\bibitem{kuti}  J.~Kuti, L.~Lin, Y.~Shen, Nucl. Phys. (Proc. Suppl.) B 4
(1988) 397; Phys. Rev. Lett. 61 (1988) 678.
\bibitem{lusc}  M.~L\"uscher and P.~Weisz, Phys. Lett. B212 (1988) 472.
\bibitem{hase}  A.~Hasenfratz et al., Nucl. Phys. B317 (1989) 81.
\bibitem{syman} K.~Symanzik, Nucl. Phys. B226 (1983) 187.
\bibitem{zimm} M.~G\"ockeler, H.~Kastrup, T.~Neuhaus and F.~Zimmermann,
 Nucl. Phys. (Proc. Suppl.) B26 (1992) 516. 
\bibitem{neub}U.~M.~Heller, H.~Neuberger and P.~Vranas, Nucl. Phys. B405
(1993) 557. 
\bibitem{einh} M.~B.~Einhorn, Nucl. Phys. B246 (1984) 75.
M.~B.~Einhorn and D.~N.~Williams, Phys. Lett. B211 (1988) 4570.
\bibitem{lang} C.~B.~Lang, Phys. Lett. B229 (1989) 97; Nucl. Phys. 
B (Proc. Suppl.) 17 (1990) 665.
%%%%%%
%%%%%%%%%%%% BOA Approximation 
%%%%%%
\bibitem{leut} A.~Hasenfratz et al., Nucl. Phys. B356 (1991) 332.
%%%%%%
%%%%%%%%%%%% Luescher's formula
%%%%%%
\bibitem{luscf} M.~L\"uscher, Nucl. Phys. B354 (1991) 531; Nucl. 
Phys. B364 (1991) 237.
\bibitem{luscwolf} M.~L\"uscher, U.~Wolff, Nucl. Phys. B339 (1990)
 222.
\bibitem{zimmph1} F.~Zimmermann, J.~Westphalen, M.~G\"ockeler and
H.~A.~Kastrup, Nucl. Phys. B (Proc. Suppl.) 30 (1993) 879.
\bibitem{zimmph2} F.~Zimmermann, J.~Westphalen, M.~G\"ockeler and
H.~A.~Kastrup, Nucl. Phys. B (Proc. Suppl.) 30 (1994) 879.
\bibitem{dewitt} B.~S.~DeWitt, Phys. Rev. 103 (1956) 1565.

\end{thebibliography}

